Discovery of ST1 centers in natural diamond

The ST1 center is a point defect in diamond with bright fluorescence and a mechanism for optical spin initialization and readout. The center has impressive potential for applications in diamond quantum computing as a quantum bus to a register of nuclear spins. This is because it has an exceptionally high readout contrast and, unlike the well-known nitrogen-vacancy center, it does not have a ground state electronic spin that decoheres the nuclear spins. However, its chemical structure is unknown and there are large gaps in our understanding of its properties. We present the discovery of ST1 centers in natural diamond. Our experiments identify interesting power dependence of the center's optical dynamics and reveal new electronic structure. We also present a theory of its electron-phonon interactions, which we combine with previous experiments, to shortlist likely candidates for its chemical structure.

==> Figures/Fig4/definitions.tex <==
% Define Colours
\definecolor{ourBlue}{HTML}{0000FF}%Blue
\definecolor{ourOrange}{HTML}{FFA400}%Orange
\definecolor{ourGreen}{HTML}{008B00}%Green
\definecolor{ourMagenta}{HTML}{FF34A7}%Magenta
\definecolor{ourPurple}{HTML}{632280}%Purple
\definecolor{ourBrown}{HTML}{5E3100}%Brown

%spin stugg
\newcommand{\ToneSpin}{\mathit{T}_1^\mathrm{Spin}}
\newcommand{\ToneOrbit}{\mathit{T}_1^\mathrm{Orbit}}
\newcommand{\cw}{\mathrm{CW}}

% color centres
\newcommand{\NV}{$\mathrm{NV}^-$}


\newcommand{\siv}{$\mathrm{SiV}^-$}
\newcommand{\SIV}{$\mathrm{SiV}^-$}
%symetry
\newcommand{\Dthreed}{\mathrm{D}_\mathrm{3d}}
%bra ket

\newcommand{\bra}[1]{$\left\langle #1 \right|$}
\newcommand{\ket}[1]{$\left| #1 \right\rangle$}

==> Figures/Fig_app1/definitions.tex <==
% Define Colours
\definecolor{ourBlue}{HTML}{0000FF}%Blue
\definecolor{ourOrange}{HTML}{FFA400}%Orange
\definecolor{ourGreen}{HTML}{008B00}%Green
\definecolor{ourMagenta}{HTML}{FF34A7}%Magenta
\definecolor{ourPurple}{HTML}{632280}%Purple
\definecolor{ourBrown}{HTML}{5E3100}%Brown

%spin stugg
\newcommand{\ToneSpin}{\mathit{T}_1^\mathrm{Spin}}
\newcommand{\ToneOrbit}{\mathit{T}_1^\mathrm{Orbit}}
\newcommand{\cw}{\mathrm{CW}}

% color centres
\newcommand{\NV}{$\mathrm{NV}^-$}


\newcommand{\siv}{$\mathrm{SiV}^-$}
\newcommand{\SIV}{$\mathrm{SiV}^-$}
%symetry
\newcommand{\Dthreed}{\mathrm{D}_\mathrm{3d}}
%bra ket

\newcommand{\bra}[1]{$\left\langle #1 \right|$}
\newcommand{\ket}[1]{$\left| #1 \right\rangle$}

==> body/trash.tex <==

\section{\label{sec:experimentalDetails} Analysis and Results}
\begin{figure}
\includegraphics{Figures/Fig1_1}
\caption{\label{fig:confocal_1}(a) Confocal fluorescence image of the natural diamond sample. (b) Resonant microwave assisted confocal fluorescence image of the same region shown in fig a. Spatially isolated color center of interest is marked in solid circles. (c) Zoomed-in confocal image of the color center at high laser power showing the characteristic doughnut response. (d) Normalized photon autocorrelation function measured at different laser power showing anti-bunching at $ \tau =0 $, which is the signature of single quantum emitters.
}\end{figure}


Figure~\ref{fig:confocal_1} (a) is a confocal imaging showing the fluorescence emitted by all defect centres in the sample. To isolate the ST1 centers, we monitored the fluorescence intensity while applying microwaves resonant with with the known ST1 spin transitions. The resulting ``ESR-assisted" confocal image is shown in Figure~\ref{fig:confocal_1} (b). The solid circles mark centers that showed a response to the applied microwave frequencies. We found that the centers were abundant in the sample and did not show particular spatial localization. The brightness of the center was comparable to that of NV centers between laser power $\approx$ \SI{100}{\micro\watt} to \SI{200}{\micro\watt} and did not exhibit blinking. At high laser power, the fluorescence of the defects decreased and showed a doughnut fluorescence pattern as shown in Figure~\ref{fig:confocal_1} (c). We also recorded a second-order photon autocorrelation characteristic of a single-photon emitter, this is plotted in Figure~\ref{fig:confocal_1} (d).


We obtained the emission spectrum at 5K because there was no discernable zero phonon line (ZPL) at room temperature; Figure~\ref{fig:Spectrum_1} shows the background-subtracted emission spectrum of a single site with a prominent ZPL around \SI{555}{nm} (\SI{2.23}{eV}) and a broad phonon side-band (PSB) extending out to \SI{750}{nm}. The fluorescence energy and narrow linewidth of the ZPL indicate that the associated electronic transition is between discrete electron orbitals within the diamond bandgap. We found that other centers in the sample show a spread of $\approx$ \SI{20}{nm} in the energy of the ZPL. The ZPL frequency distribution is inset as a histogram in Figure~\ref{fig:Spectrum_1}. Since all the measured defects show similar zero field splitting parameters, we attribute the distribution of ZPL to the strain in the local environment of the defect. This also supports the established electronic configuration for the ST1 center [REFERENCE], where the main transition is between the singlet states and the ESR is observed by manipulating a photoexcited triplet state.

%\subsection{\label{sec:citeref}Magnetic dipole orientation}
Figure~\ref{fig:magnetic_dipole_orientation} (a) shows the response of fluorescence intensity while sweeping the microwaves from \SI{200}{MHz} to \SI{1,400}{MHz}. We observed three distinct peaks in fluorescence intensity at microwave frequencies centered at approximately \SI{220(1)}{MHz}, \SI{990(1)}{MHz} and \SI{1.280(1)}{GHz}. These resonances are consistent with studies of the ST1 recorded by \citet{lee_2013_ST1}.

Enhanced fluorescence under the influence of the resonant microwave field is a well-studied phenomenon for fluorescent molecule, and molecule-like defects, consisting of singlet ground and excited states with an additional triplet shelving state\cite{Chiha_1964_ODMR,Brown_1994_ODMR,Angerhofer_1994_ODMR}. If the system has low symmetry, the dipolar spin-spin coupling between the unpaired electrons lifts the threefold degeneracy of the triplet state. Under continuous optical illumination the triplet sublevels ($\text{T}_\text{(0,-,+)}$) are populated from the excited singlet state due to finite spin-orbit coupling. The transition probabilities and symmetry selection rules often favour accumulation of population in the triplet manifold. This ultimately leads to spin-polarization into the triplet sublevel with the longest lifetime. Application of resonant microwave fields to mixes the spin population between the sublevels. This results in an increase in the probability fluorescent transitions to the ground state. 

\todo{Current Changes Up to Here}

Such electronic triplet states being paramagnetic, serve as an intrinsic spin probe of the system, and its interactions with the environment. The spin-Hamiltonian describing the fine structure of the triplet level is of the form\cite{Loubser_1978_ESRdiamond}, 
\begin{align}
\hat{H}=D\left[S^2_z-\frac{1}{3} S (S+1)\right]+\overset{\rightharpoonup }{S}.g.\overset{\rightharpoonup }{B}+E \left(S^2_x-S^2_y\right)
\label{eq:Hamiltonian}
\end{align}
where$\overset{\rightharpoonup }{S}$ spin operator,$\overset{\rightharpoonup }{B}$ is the magnetic field vector, D and E are zero field splitting parameters g is the isotropic g factor.Note that the Hamiltonian is written in the defects coordinate system where the crystal field tensor D is diagonalized.The two peaks observed in \ref{fig:confocal_1} can be assigned to the resonant transitions between $T_{\text{0}} \Longleftrightarrow T_{\text{+}}$ and $T_{\text{0}} \Longleftrightarrow T_{\text{-}}$ respectively, yielding the zero field splitting parameter of D $\approx$ 1130(5) MHz and  E $\approx$ 135(5) MHz.
%The resonance between $T_{\text{+}} \Longleftrightarrow T_{\text{-}}$ is observable, though not always measured due to our hardware limitation.
The zero field splitting parameters D and E represent spatial distribution of electron and commonly are sensitive to the local electronic distortions introduced by the environment.
However the measured values of D and E are fairly constant over several defects, strongly suggesting that the presence of large E parameter is indeed due to the low symmetry of the defect\cite{Loubser_1978_ESRdiamond}.
In order to identify the orientation of the magnetic main axes, the spin transition frequencies are recorded while rotating the magnetic field of magnitude $\approx$ 120 G,in the plane perpendicular to [001] axis.
\begin{figure}
\includegraphics{Figures/Fig3}
\caption{\label{fig:magnetic_dipole_orientation}(a) Optically detected magnetic resonance spectrum of the colour center at zero magnetic field.(b)Angular response of the ESR transition frequencies(D+E,D-E)when B=120 Gauss is rotated in the [001] crystal plane.The solid line represent the fit using \eqref{eq:Hamiltonian}.
}
\end{figure}

In figure\ref{fig:magnetic_dipole_orientation}a dots represent the measured spin transition frequency and the solid line are simulated curves calculated by the numerical diagonalization of the spin Hamiltonian given in equation \ref{eq:Hamiltonian} for a triplet state with $\langle$110$\rangle$ orientation.The simulated curves well reproduce the major features of the experimental results, suggesting that the major symmetry axis of the defect is along the $\langle$110$\rangle$ crystal direction with the minor axes in the plane orthogonal to the corresponding $\langle$110$\rangle$ vector(e.g x $\parallel$ [100], y $\parallel$ [011], z $\parallel$ [01$\overline{1}$]).The apparent deviation between the measurement and simulation specially when the magnetic field is perpendicular to the defects's main axis, strongly suggests the possibility of a slight tilt from the predicted direction of the defect's minor axes.The estimation of this projection angle is hindered by the broad linewidth of the signal.
%However there is a possibility that the defect's minor axes slightly tilt from the predicted crystal axes, because the linewidth of the signal was too broad to estimate the projection angle accurately.
The measured direction of the center's major symmetry axis and predicted low symmetry is consistent with the reported ST1 center\cite{lee_2013_ST1}.It should be stressed that none of the measured defects showed intrinsic hyperfine coupling.This excludes the presence of nitrogen from the defect structure, which is the dominant impurity in most diamond crystals.
From the fact that the defect's major symmetry axis is along the $\langle$110$\rangle$ direction ,it seems likely that the defect structure involves impurity atoms and/or vacancies occupying several lattice sites coplanar in the (110) plane.
%Since the defect is observed even deep inside the diamond, the involvement of transition-metal impurity is less favorable.%
The role of oxygen as impurity in the defect structure is highly suspicious,with a possible structure of O-C-O v-O-v in the (110) plane.
\begin{figure}
\includegraphics{Figures/Fig5_1}
\caption{\label{fig:Optic_dipole_orientation} Measured polarization dependent emission, showing four fold symmetry pattern.
}
\end{figure}

Figure\ref{fig:Optic_dipole_orientation} shows the polar plot of the fluorescence intensity,revealing the existence of four linear polarization states, defined as  $\phi_1 = 0\degree$, $\phi_2=45\degree$,  $\phi_3=90\degree$ and $\phi_4=135\degree$.
This four fold symmetry on the projected [001] plane strongly suggest that the dipoles are oriented along the $\langle$110$\rangle$ crystal direction. Of the six possible$\langle$110$\rangle$ orientations, two are degenerate when projected on the [001] axis. At this point we are unable to find any correlation between the optical and magnetic dipole orientation.
%\subsection{Photodynamics}
%\begin{figure}[h]
%\includegraphics[width=0.8\textwidth]{pictures/level_scheme_3}
     %\caption{(a)Level scheme.(b)Triplet sublevel.}\label{fig:lvl}
%\end{figure}
\begin{figure*}
\includegraphics{Figures/Fig4}% Here is how to import EPS art
\caption{\label{fig:fluorescence}(a)Extended level scheme to account for the fluorescence saturation behaviour.(b)Measured fluorescence counts as a function of increasing pump power.(c)Measured ODMR contrast as a function of increasing pump power.(d)Extracted triplet depopulation rates.(e) 
}
\end{figure*}

The unique photoluminescence property that marks the colour centers apart from the background defects is the phenomenal drop in their steady state fluorescence with respect to increasing pump power which is shown in Fig\ref{fig:fluorescence}(b). NV centers also show similar behavior, which is attributed to photoionisation of the excited electron to the dark $\text{NV}^0$ state via excited state assisted transition 
\cite{Waldherr_2011_Dark_States}. However in case of the colour center, the decreasing fluorescence trend is not followed by the ESR contrast,thus eliminating the possibility of the excited electron to be trapped by a donar, but rather pumping it to the triplet sublevels, ultimately leading to a high degree of polarization of the triplet states. Experimentally with high laser power a contrast of $\approx$ 80$\%$ is measured.

The  purpose  of  this section  is  to  revisit  our  present understanding of the defect's dynamics under optical excitation and to provide a minimalist explanation for the observed behavior.The simplest electronic structure that could account for the observed enhancement in fluorescence under resonant microwave field is with singlet ground and excited states and additional triplet shelving states with different depopulation rates depending on its spin projection. The dynamics of such system under optical excitation can be described as rate equations\cite{Vries_1979_Fluorescence_transient}\cite{Bernard_1993_probe_for_intersystem}\cite{Brown_1994_ODMR}.

\begin{align}
\begin{split}
\dot{S_{\text{S0}}} &= -k_{\text{ex}} S_{\text{S0}}+k_f S_{\text{S1}}+T_0 k_{T_0}+T_- k_{T_-}+T_+ k_{T_+} \\
\dot{S_{\text{S1}}} &= k_{\text{ex}} S_{\text{S0}}-k_f S_{\text{S1}}-k_{\text{ISC}} S_{\text{S1}} \\
\dot{T_+} &= \frac{k_{\text{ISC}}}{3} S_{\text{S1}}-T_+ k_{T_+} \\
\dot{T_-} &= \frac{k_{\text{ISC}}}{3} S_{\text{S1}}-T_- k_{T_-}\\
\dot{T_0} &= \frac{k_{\text{ISC}}}{3} S_{\text{S1}}-T_0 k_{T_0}\\
\end{split}
\label{eq:5LS}
\end{align}
Such a system is known to exhibit saturation of fluorescence which is governed by rate of trapping to the metastable triplet state and the depopulation rate of the state. The assumption that the triplet states share the same inter-system crossing rate $ k_{ISC} $ is made for the sake of simplicity. In reality, the rate of populating/depopulating the triplet state is determined by the defect's symmetry and therefore differ for different spin projections. In order to gain further insight into the time dependent kinetics of the system, second order correlation function is measured on single spots with Hanbury Brown and Twiss (HBT) configuration. The intensity autocorrelation function is defined as the probability of detecting a pair of photon during t and t+$\tau$ which is proportional to the probability of occupying the excited state with the conditional probability to occupy the state at t+$\tau$ starting from the ground state at t. In other words, it is the transient solution of eqn. \ref{eq:5LS} for the excited state $S_{\text{S1}}$. Using the conservation of total population, one equation and one variable has been eliminated from equation 2. The solution of the resulting equation can be found after Laplace transformation and the correlation function as sum of complex exponentials is given as
\begin{equation}
\begin{split}
g_2(\tau)=1-\alpha e^{-\lambda_1 t}-\beta e^{-\lambda_2 t}-\gamma e^{-\lambda_3 t}-\delta e^{-\lambda_4 t}
\label{eq:g_2_fit}
\end{split}
\end{equation}
where $\lambda_1,\lambda_2,\lambda_3,\lambda_4$ are the roots of the cubic characteristic equation.
Two important features to note in Fig.\ref{fig:fluorescence} are the anti-bunching seen at $ \tau =0 $, which is the signature of single quantum emitters and the prominent bunching at $ \tau < 0 $, which reveals the existence of a shelving state. Using equations \ref{eq:5LS} and \ref{eq:g_2_fit}, it is possible to express the rates $ k_{x} $ in terms of the fit parameters of the measured $ g_2(\tau) $ function. The actual mathematical derivation of the individual rates $ k_{x} $ is fairly straight forward and given in the appendix.%
Here we only focus on the behavior of the extracted rates with respect to the excitation power which is shown in Fig. \ref{fig:fluorescence}c.
It can be seen from Fig.\ref{fig:fluorescence} that the depopulation rate of the triplet sublevels $ k_{T_0} $, $ k_{T_-} $ and$ k_{T_+} $ are not influenced by the increase in the pump rate. This eliminate the possibility of any intensity dependent depopulation channel from the triplet manifold. The dashed lines in Fig.\ref{fig:fluorescence} marks the values of these rates ($ \frac{1}{k_{T_0}} \approx $ 2120 ns  and $\frac{1}{ k_{T_-}} \approx$  440 ns)  measured aprori using the method described in \cite{lee_2013_ST1}. Fig.\ref{fig:fluorescence} shows that $k_{ex} $ increases linearly with the excitation power, while $k_{f} $ remains constant. This behavior fits well with the physical description of these parameters, where $ k_{f} $ the spontaneous emission rate is dictated only by Fermi's golden rule and the relation between $ k_{ex} $ and $ P_{ex} $ is given in eqn \ref{eq:kex_to_power}\todo{Missing equation reference}. From the slope of the measured $ k_{ex} $ we estimate the absorption cross section $\sigma \approx 10^{-17} cm^2 $ which is similar to the reported absorption cross section of NV center at 532nm in a 1b diamond. The power dependence of the intersysten crossing rate $ k_{ISC} $ plotted in Fig.\ref{fig:fluorescence} is quite unexpected. The linear increase of $ k_{ISC} $ with the excitation power strongly suggest the presence of a non-radiative intensity dependent transfer of the excited state population. Excited state absorption or two photon absorption to a higher excited state is a possible explanation. An extended level scheme is shown in the figure, where the process of excited state absorption is included. Since its is impossible to find analytical solutions for such system, the influence of the excited state absorption is included phenomenological in eqn. \ref{eq:5LS} with the assumption that lifetime of the higher excited states are very small. As shown in the appendix, the slope of the of $ k_{ISC} $ vs  $ P_{ex} $ give the cross section of excited state absorption which is $\sigma_{ESA} \approx 10^{-19} cm^2 $. This model along with the estimated values of the rates and the corresponding absorption cross-section, fits well with the observed steady-state fluorescence. The blue dashed line in Fig.\ref{fig:fluorescence} is the fit using the extended model, where the absorption cross-sections were free parameters.
%The extracted values match well with the previously estimated values absorption cross-sections.
In the following we shortly summarize the source of errors in the estimation of the rates.The consequence of the errors in the evaluation of the fit parameters of the $g_2(\tau)$ function is quite significant in the estimation of the rates. At low power, weak bunching makes the estimation of estimation of the triplet life-times quite challenging.Uncertainty in both the pre-exponential term and decay time translates to uncertainty in  these rates.In high power regime, where the defects fluorescence decrease, careful background correction is needed.Though the extracted values of different population/depopulation rates and the absorption cross-section suffer from the limitations of data evaluation, the presented model gives a minimal theoretical description of the experimentally observed behavior.The manifestation of this intensity dependent shelving to the dark state is seen quite remarkably in the confocal image.
% a rapid (~1/70 ns) inter-system-crossing rate from the singlet excited state to the triplet state and
% substantial differences among the triplet lifetimes, τ|0⟩≈2500 ns, τ|-1⟩≈1000 ns, τ|+1⟩≈200 ns. These are
% responsible for the positive and exceptionally high (45 \%) optical spin signal contrast, and increasing

% steady-state fluorescence response to a randomly aligned static magnetic field as observed in Fig. 1d
% because mixing the triplet sublevels results in faster decay to the ground state. It follows that optical
% pumping prepares the system in a spin polarized state of the meta-stable triplet state with predominant
% population of the slowly decaying triplet sublevel, |0⟩.
% The key features of the ST1 optical cycle are: 
% A key feature of the defect is that its state can be optically spin-polarized and read out. During the optical cycle, the state may either 

% We now show the application of the metastable electron spin as a universal single nuclear spin gate and
% demonstrate coherent manipulation and readout of the nuclear spin in the spin-free electronic ground
% state.

% The electron spin is polarized because the excited state may undergo a spin-projective dark transition to a long lived triplet sublevel. 


% The optical cycle of the ST1 exhibits a dark transition from the excited to the ground state. This transition occurs via intersystem crossings (ISCs) to and from the triplet level. Since ISCs are allowed by spin-orbit coupling and mediated by phonon emission, the transitions are dependent on the triplet's spin projection.

% The optical cycle of the ST1 starts by excitation of an electron from the ground singlet to a vibronic state of the excited singlet. The state then quickly decays non-radiatively through the vibronic levels. After this, the defect then either radiatively decays back to the ground state or non-radiatively transitions to the metastable triplet via an intersystem crossing (ISC). The defect decays from the triplet to the ground state by a subsequent ISC. Since the ISCs are allowed by spin-orbit coupling and mediated by phonon emission, the ISCs rates are dependent on the triplet spin-projection. 

% The NV− centre may also be identified by a zero field magnetic resonance at ∼2.88 GHz [44, 45] (see figure 3). This magnetic resonance occurs
% between the ms = 0 and ms = ±1 spin sub-levels of the spin triplet ground
% state 3A2 and can be detected by either conventional electron paramagnetic
% resonance (EPR) [44, 45] or optically detected magnetic resonance (ODMR)
% [78] techniques. A further ODMR at ∼1.42 GHz [79, 80] is observed at room
% temperature (see figure 3) and is attributed to a zero field splitting of the
% electron g-factors ∼2.0028 [44, 45] and ∼ 2.01 [79] respectively. The magnetic resonances of 3A2 [81, 82] and 3E [79, 80] also exhibit weak interactions
% with strain and electric fields
% spin triplet excited state 3E that is analogous to that of 3A2. The magnetic
% resonances of 3A2 and 3E behave as would be expected of triplet spins in
% a trigonal crystal field and are characterised by the approximately isotropic
% At low temperatures (<10 K), the excitation spectrum of the NV− optical ZPL (refer to figure 3) reveals a fine structure of the ZPL that is highly
% dependent on strain [84] and electric fields [85]. The fine structure of the ZPL
% implies a fine structure of 3E that is much more complicated than that suggested by the associated ODMR at room temperature. The low temperature
% fine structure of 3E and its observed dependence on strain [84] is depicted
% in figure 4 (analogous results have been obtained using electric fields [85]).
% It is clear that the presence of strain and/or an electric field splits the 3E
% fine structure into two branches; the lower branch undergoes two level anticrossings (as marked in figure 4) that mix the lower fine structure states to a
% degree dependent on the strain/electric field, whereas the upper branch does
% not experience any level anti-crossings and the upper fine structure states
% remain approximately unmixed [85]. The mixing of the lower fine structure
% states results in optical spin-flip transitions when the lower branch is excited,
% states (believed to be 1A1 and 1E) [47, 89, 90]. As these non-radiative decay pathways compete with fluorescent decay, the spin projection with the
% weakest non-radiative decay out of 3E will appear brightest and vice versa


% To isolate the ST1 centers, we monitored the fluorescence intensity while applying microwaves resonant with with the known ST1 spin transitions. The resulting ``ESR-assisted" confocal image is shown in Figure~\ref{fig:confocal_1} (b). We found that the centers were abundant in the sample and did not show particular spatial localization. The brightness of the center was comparable to that of NV centers between laser power $\approx$ \SI{100}{\micro\watt} to \SI{200}{\micro\watt} and did not exhibit blinking. At high laser power, the fluorescence of the defects decreased and showed a doughnut fluorescence pattern as shown in Figure~\ref{fig:confocal_1} (c). We also recorded a second-order photon autocorrelation characteristic of a single-photon emitter, this is plotted in Figure~\ref{fig:confocal_1} (d).

% We obtained the emission spectrum at 5K because there was no discernable zero phonon line (ZPL) at room temperature; Figure~\ref{fig:Spectrum_1} shows the background-subtracted emission spectrum of a single site that is consistent with the ST1. We found that other similar centers in the sample show a spread of $\approx$ \SI{20}{nm} in the energy of the ZPL. The ZPL frequency distribution is inset as a histogram in Figure~\ref{fig:Spectrum_1}. Since all the measured defects show similar zero field splitting parameters, we attribute the distribution of ZPL to the strain in the local environment of the defect. 
